Efficient Attribute Unlearning: Towards Selective Removal of Input Attributes from Feature Representations

Recently, the enactment of privacy regulations has promoted the rise of the machine unlearning paradigm. Existing studies of machine unlearning mainly focus on sample-wise unlearning, such that a learnt model will not expose user's privacy at the sample level. Yet we argue that such ability of selective removal should also be presented at the attribute level, especially for the attributes irrelevant to the main task, e.g., whether a person recognized in a face recognition system wears glasses or the age range of that person. Through a comprehensive literature review, it is found that existing studies on attribute-related problems like fairness and de-biasing learning cannot address the above concerns properly. To bridge this gap, we propose a paradigm of selectively removing input attributes from feature representations which we name `attribute unlearning'. In this paradigm, certain attributes will be accurately captured and detached from the learned feature representations at the stage of training, according to their mutual information. The particular attributes will be progressively eliminated along with the training procedure towards convergence, while the rest of attributes related to the main task are preserved for achieving competitive model performance. Considering the computational complexity during the training process, we not only give a theoretically approximate training method, but also propose an acceleration scheme to speed up the training process. We validate our method by spanning several datasets and models and demonstrate that our design can preserve model fidelity and reach prevailing unlearning efficacy with high efficiency. The proposed unlearning paradigm builds a foundation for future machine unlearning system and will become an essential component of the latest privacy-related legislation.

==> sections/Approximation.tex <==
\section{Approximate Disentanglement}

Since $I(h,r^*)$ and $I(h, s^*)$ are difficult to calculate in practice, we use the upper bound of the function (\ref{original loss func}) to approximate the loss. Our result is in the Proposition \ref{approximate loss}, with the detailed proof below. For convenience, we will omit the subscript of loss in the following part.
% \newtheorem{proposition}{Proposition}
\begin{proposition} \label{approximate loss}
Suppose that the Markov chain $(y,r, s)\rightarrow \boldsymbol{x}\rightarrow \boldsymbol{h}$ holds. Then the upper bound of $\mathcal{L}$ is as follows
\begin{eqnarray}
    \mathcal{L} \le -\lambda_1I(\boldsymbol{h},\boldsymbol{x})-\lambda_2I(\boldsymbol{h},y)-\lambda_3I(\boldsymbol{h},z) \nonumber 
    =\overline{\mathcal{L}}
\end{eqnarray}
where $\lambda_1=\alpha(1-\beta)$, $\lambda_2=\alpha\beta$, $\lambda_3=\alpha(\beta-\gamma)$, $\beta\geq\gamma$, and $z$ represent the sensitive attribute.
\end{proposition}
Suppose $\gamma>\beta$, the blur of the sensitive information possibly contains much information critical to the recognition, which would degrade the recognition accuracy. We intend to conceal the sensitive information instead of devastating the recognition. Compared with the level of removing the background or irrelevant information, the blur degree of sensitive information should be mild.

To guarantee the accuracy of approximation, the gap between $\mathcal{L}$ and $\overline{\mathcal{L}}$ should be small. We present a bound of the gap in the Proposition \ref{gap}.
\begin{proposition}\label{gap}
Assume that there exists a deterministic function map $x$ to $y$, the gap $\epsilon=\overline{\mathcal{L}}-\mathcal{L}$ can be bounded by
\begin{equation}
    \epsilon \le \alpha\beta(I(\boldsymbol{x},y)-I(\boldsymbol{h},y)-I(\boldsymbol{h},z))
\end{equation}
\end{proposition}
According to the conclusion of mutual information estimation \cite{Wang2021revisiting}, we can calculate $I(h,\boldsymbol{x})$ by $R_w(\boldsymbol{x}|\boldsymbol{h})$ which is the expected error for reconstructing $\boldsymbol{x}$ from $\boldsymbol{h}$, and as for $I(\boldsymbol{h},y),I(\boldsymbol{h},z)$,  we can train auxiliary classifiers $q_{\psi_1}(y|\boldsymbol{h}),q_{\psi_2}(z|\boldsymbol{h})$ to approximate.
%\subsection{Asynchronous Training}
% To further accelerate training procedure, local update is used to facilitate the SL training. Previous SL paradigms normally update both client and server's parameters in a sequential order, which can cause a serious delay due to the backward locking, since neither side can be updated before receiving gradients from another one, which means that only one of the participants is active at the single time slot.

% As a comparison, \SysName{} is more efficient for the asynchronous training. After processing the input images with client model, parameters can be updated locally using the Information Filtration Loss $L_{infoFiltra}$, without waiting for the gradients coming from server starting from the bottom layer. Meanwhile, intermediate features transmitted to the cloud can update server parameters simultaneously. In this way, client and server can work simultaneously, as shown in Fig.~\ref{fig:asy}.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/asy.png}
%   \caption{\textbf{Asynchronize}: Edge device and server work asynchronously in training model in a parallel way. }
%   \label{fig:asy}
% \end{figure}




==> sections/Definition.tex <==
\section{Define Vertical Machine Unlearning}\label{sec:Define}
To better understand the problem and meet the requirements of \textit{the right to be forgotten}, we identify two challenges which is unique in the context of vertical unlearning. Then we give formal definition of vertical unlearning problem by revisiting challenges during the process. By overcoming these challenges, we clarify the objective vertical unlearning need to obtain in the end.

\subsection{Challenges in Vertical Unlearning}
%\hspace{\parindent}
\textbf{Feature is embedded}
Unlike the existing data sample-oriented unlearning where the target required to be forgotten is independent with each other, vertical unlearning on the other hand does not have such advantage. In the context of vertical unlearning, the objective that need to be removed, i.e., feature, is embedded in input data, which is difficult to separate them even in the data input procedure, especially in the unstructured data type, e.g., images, video. Thus, it is challenging to find a general solution to this problem like existing horizontal unlearning, since purely eliminating a subset of data samples from input source and retraining the whole model is not an option. The key reason is feature entangle with each other from the view of input space. 

\textbf{Feature is interactive} During the training process, features in the latent space interact with each other and contribute to the final model performance. So it is difficult to forget some selected sensitive features and retain the other features intact. For example, assuming a face recognition model and data holders are concerned about the race attribute being exploited for malicious use. So they require the learnt model to forget their race attribute, since they are entitled to have control over the data they provided, according to \textit{the right to be forgotten}. However, race related attributes are closely related to the model main task. So, the key challenge here in vertical unlearning is how to forget the selected attributes to the large extent with the minimized collateral damage to the other features and model performance.

\subsection{Formalizing the problem of Vertical Unlearning}
We formalize the problem of vertical unlearning as a game between two entities: 1)a trustful service provider \textit{S} with control over training process, data collection and management of whole model, 2)Data holders, who provide individual data to service provider \textit{S} for training and validating. 

Suppose we have $n$ data holders $C=\{C_1,C_2.\dots,C_n\}$, with $k$ features. let $D=\{d_1,d_2,\dots,d_n\}$ be dataset space that model train on and $F=\{f_1,f_2,\dots,f_k\}$ be the latent feature space that data space can mapping to $D \rightarrow F$, $\phi$ be the model in hypothesis space after training. Within a finite time period, service provider $S$ is required to return a model after unlearning of feature $f_u$.
% \begin{definition}[Horizontal Machine Unlearning]
%  We define the algorithm \textit{L: D $\to$ $\phi$} be a learning process which maps dataset $D$ into the hypothesis space of model $\phi$. $d_i$ be the data point that user $i$ requires to delete. We define a unlearning process \textit{U: L(D) $\otimes$ D $\otimes$ $d_i$ $\to$ $\phi$ }, which takes an input dataset $D$, a learnt model $L(D)$ and data point $d_i$ that required to be deleted. Our goal is to achieve the same probability distribution of our unlearning process of the model as the one with directly removed the instances from dataset $D$ and with good performance. Thus the objective of Horizontal Machine Unlearning can be described as the following formula:
% \begin{equation}
%     \textit{P( L( D $\backslash$ $d_i$)) = P( U( L(D), D, $d_i$))}
% \end{equation}
% where $D \backslash d_i $ defines the data samples without data point $d_i$.
% \end{definition}

\begin{definition}[Vertical Machine Unlearning]
 We define the algorithm \textit{L: F $\to$ $\phi$} be a learning process which maps latent feature space $F$ into the hypothesis space of model $\phi$. $f_u$ be the latent feature that data holders require to delete. We define a unlearning process \textit{U: L(F) $\otimes$ F $\otimes$ $f_u$ $\to$ $\phi$ }, which takes an input 
latent feature space $F=\{f_1,f_2,\dots,f_k\}$, a learnt model $L(F)$ and the feature $f_i$ that required to be forgotten. Thus the objective of Vertical Machine Unlearning can be described as
\begin{equation}
    \textit{P( L( F $\backslash$ $f_u$)) = P( U( L(F), F, $f_u$))},
\end{equation}
where $F \backslash f_u $ defines the latent feature space without selective sensitive feature $f_i$. $P(\cdot)$ denotes the distribution of models using vertical unlearning algorithm and the equation of $P(\cdot)$ indicates to have the identical distributions of each model. 
% Assuming that we are solving the problem of a supervised learning task, we also need to satisfy the task performance after unlearning selective features from the learnt model. 
\end{definition}

We also depict the architecture of horizontal learning and vertical learning in Fig.~\ref{fig:MU} to better understand the difference between the two modes. We can see from the figure that the horizontal axis represents the input space, the vertical axis represents latent feature space and each sample contains several latent features inside the data. The comparison manifests the intrinsic difference between them is that the horizontal unlearning aiming to unlearn models by deleting certain data samples while vertical unlearning targets on the features. 



% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/VMU1.pdf}
% ~  \caption{\textbf{Vertical Machine Learning}: Edge devices with limited resources leverage powerful computation resources on cloud, but may introduce information leakage when encountering malicious attacker. }
%   \label{fig:VMU}
% \end{figure}

\subsection{Goals of Vertical Unlearning}
To better comply with GDPR demand and \textit{the right to be forgotten}, we propose several goals that vertical unlearning need to meet:

\textbf{G1. Efficacy Guarantee.} Any strategy of vertical unlearning should be directed towards that the selected feature has been forgotten to the large extent. Since unlike data samples which is concrete and separate, there is no easy way to estimate the unlearning degree of selected feature. Thus, in the later session, we will introduce a general metrics to make sure that selected feature can not be exploited after vertical unlearning.

\textbf{G2. Fidelity Guarantee.}
It is obvious that model performance will be affected if feature selected to be forgotten, since features during the training are interactive with each other. Thus there exist a trade-off between the efficacy the model unlearn and the fidelity it preserved. The optimal effect is to achieve minimum gap in fidelity preserved in comparison between the model before unlearning.

\textbf{G3. Unlearning Speedup.}
\label{goal:G3}
Additionally, vertical unlearning should take the unlearning efficiency into consideration. Besides achieving decent performance, unlearning time should be reduced as far as possible at the meantime or at least no slower than naive retraining. Furthermore, to accord with this goal, we come up with a speed up strategy to accelerate the unlearning process.

\textbf{G4. Model Agnostic.}
%
The unlearning solution for vertical unlearning should be general, which means that the aforementioned goals ought to be satisfied by any model when performing vertical unlearning strategy. 


==> sections/Preliminary.tex <==
\section{Preliminaries}\label{sec:Preliminaries}
For sake of completeness, we briefly review current emerging data privacy legislation, challenges for existing machine unlearning researches and our interpretation for future machine unlearning.
%For sake of completeness, we now briefly review the collaborative learning, correspondent problems of latent feature leakage, protection methods and the threat model.

\subsection{Data Privacy Legislation}
The rapid development of Big Data boosts the advancement of Deep Learning by utilizing a massive amount of data generated from different sources across a wide range of sectors, such as healthcare and finance. Yet the risk of privacy violation increases as we savoring the benefits of 'free' data. To address the privacy issue, numbers of privacy-preserving mechanisms \cite{mehmood2016protection,papernot2016towards,liu2021machine} emerge for privacy protection at different stages from data generation to data processing. Furthermore, privacy regulation \cite{mantelero2013eu,web:lang:CCPA,garcia2020lei,de2014protection} has been introduced to legitimize and protect sensitive information against hackers and leaks to make our digital environment safer and more secure. However, more and more emerging legislation emphasizes customers' rights other than merely keeping data safe from unauthorized access. Customers have rights to control their usage permission of their information and the for what purpose. 
% Thus, Machine Unlearning arises.

% \subsection{Attribute Inference Attack}
% Although aiming at a specific task, personal data trained for deep learning models may contain other sensitive information that can be exploited. Attribute Inference Attack \cite{pasquini2021unleashing,mireshghallah2020privacy} aims at inferring sensitive attributes such as gender, ethnicity from a given learnt model with the exposure of non-sensitive attribute and intermediate model output. In general, the attacker trains on an adversarial network with non-sensitive attributes and intermediate output as model input and then leverages the trained model to infer the hidden sensitive attributes inside the user private data \cite{jia2018attriguard}.

% \subsection{Existing Protection}
% We characterize existing protection against the sensitive attribute leakage into three categories: (1) adding noise or blurring to the raw data; (2) combining the learning with cryptographic techniques; (3) directly removing sensitive information out of models.
% %
% The protection of the first two categories are general-purpose protection which could be broadly applicable across privacy domains.
% %
% However, obfuscating sensitive information by adding noise or blurring is ineffective against deep neural network based adversarial attacks \cite{ren2018learning,osia2020hybrid,oh2016faceless,liu2021adversarial}.

% Cryptographic techniques, e.g., homomorphic encryption and secure multi-party computation can protect the latent features from being exposed to any external parties including the server as training is performed on ciphertexts or satisfying zero-knowledge proof.
% %
% But these techniques incur unacceptable overhead to computation and communication \cite{zhang2020batchcrypt,so2021turbo}.
% %
% Hardware accelerator can be applied to ease such overhead \cite{reagen2021cheetah}, however, using dedicated hardware sacrifices the generality and the further application scope, leading to undesirable trade-off. 

% Compared to general-purpose protection as above, the latest study provides another viewpoint from which the sensitivity information are directly removed out of models.
% %
% It learns a channel pruner to selectively prune channels which leak sensitive information.
% %
% The output of channel pruning are binary i.e., 0 or 1 in nature, where 0 deactivates channels that contribute to sensitive information \cite{singh2021disco}.


\subsection{Challenges in Existing Machine Unlearning}
To cope with the \textit{the right to be forgotten} appeal in recently brought up legislation, the European Union's General Data Protection Regulation (GDPR) \cite{mantelero2013eu}, another branch of privacy-preserving Machine Learning arised, called Machine Unlearning \cite{cao2015towards,bourtoule2021machine}. Machine Unlearning is brought to address the challenges of unlearning required data samples from a learnt model without compromising previous model performance. As the development of this field goes on, several research variants emerged. One of the factions eyes on the enormous computational overhead during the process and focus on promoting unlearning efficiency \cite{huang2021unlearnable,sekhari2021remember,gupta2021adaptive,brophy2021machine}, another direction aiming at pushing this technique into extensive scenarios, e.g., recommendation system, federated learning, lifelong learning \cite{chen2022recommendation,wang2022federated,shibata2021learning}. However, although achieving much progress, none of these works innovating from source, i.e., the unlearning objective. Since the existing techniques focus on the perspective from horizontal dimension, i.e, data samples space, we define it as horizontal unlearning. 
%\cite{cao2015towards} first introduced the term "Machine Unlearning" and proposed an possible way to solve it. After that, \cite{bourtoule2021machine} proposed a sharding-based strategy leveraging ensemble learning and distributed manner, which establish a general method and a new baseline for further research. Later studies either focus on the different algorithms or minimizing computational and storage complexity in this area \cite{huang2021unlearnable,sekhari2021remember,gupta2021adaptive,brophy2021machine}.



\subsection{Envision for Future Machine Unlearning}
%
Emergent privacy protection not only focus on protecting data from unauthorized access, but also concerning subjective intention of how their data be used and what the purpose of utilization.
%
Most of the studies have an eye on addressing this issue by unlearning data samples from the learnt model, however, such action only handles the problem from data space level and might severely influence the model performance especially when the data samples that required to be deleted enlarging.
%
We interpret the machine unlearning from the orthogonal perspective, i.e., to eliminating personal information from latent feature space in the vertical direction. This particular thoughts can either satisfy the protection of certain sensitive features, e.g. gender, ethnicity, but also retain the contribution to the model learned from these data samples.  


% \subsection{Collaborative Learning}
% Centralized learning is sometimes not a good option because users are not willing to share raw data \cite{liu2021machine}.
% %
% In this case, ML can be conducted in a collaborative manner, in which each user trains the network up to a certain layer known as the cut layer and sends the intermediate activations to server. 
% %
% Formally, these activations represent and compress the input data to some intermediate feature vectors known as feature maps.
% %
% The server then trains the network for rest of the layers, and generates the gradients for the final layer, followed by error back-propagation until the cut layer.
% %
% The gradient is then passed over to the users. 
% %
% The rest of the back-propagation is completed by the users \cite{poirot2019split}.

% \subsection{Latent Feature Leakage}
% Although collaborative learning provides default privacy by sharing intermediate activations instead raw data to server, recent studies have noted that shared activations still leak latent features \cite{zhao2020trade,liu2019privacy,pasquini2021unleashing,roy2019mitigating,bertran2019adversarially}. 
% %
% They have attempted the related attacks of feature extraction by focusing on adversarial representation learning (ARL).
% %
% These attacks may identify and quantify bias in datasets by an adversarial network aiming to maximize the extraction of sensitive information from a given intermediate activation. 
% %
% The bias routinely manifests as some attributes of the input, e.g., age, race, gender for facial images.

% \subsection{Existing Protection: Limitations}
% We characterize existing protection against the latent feature leakage into three categories: (1) adding noise or blurring to the raw data; (2) combining the learning with cryptographic techniques; (3) directly removing sensitive information out of models.
% %
% The protection of the first two categories are general-purpose protection which could be broadly applicable across privacy domains.
% %
% However, obfuscating sensitive information by adding noise or blurring is ineffective against deep neural network based adversarial attacks \cite{ren2018learning,osia2020hybrid,oh2016faceless,liu2021adversarial}.

% Cryptographic techniques, e.g., homomorphic encryption and secure multi-party computation can protect the latent features from being exposed to any external parties including the server as training is performed on ciphertexts or satisfying zero-knowledge proof.
% %
% But these techniques incur unacceptable overhead to computation and communication \cite{zhang2020batchcrypt,so2021turbo}.
% %
% Hardware accelerator can be applied to ease such overhead \cite{reagen2021cheetah}, however, using dedicated hardware sacrifices the generality and the further application scope, leading to undesirable trade-off. 

% Compared to general-purpose protection as above, the latest study provides another viewpoint from which the sensitivity information are directly removed out of models.
% %
% It learns a channel pruner to selectively prune channels which leak sensitive information.
% %
% The output of channel pruning are binary i.e., 0 or 1 in nature, where 0 deactivates channels that contribute to sensitive information \cite{singh2021disco}.





%Traditional methods focus on protecting the input data by adding noise or blurring \cite{ren2018learning,osia2020hybrid,oh2016faceless} to obfuscate some exclusive features. However, these methods are ineffective against DNN-based Adversarial Attacker\cite{liu2021adversarial} and show unsatisfactory performance. 

%Another way of protecting the intermediate features is to use the Homomorphic Encryption \cite{brakerski2014leveled}. However, such complicated encryption and decryption procedure may lead to excessive extra latency, which is not adequate when performing inference since instant response is demanded. Hardware accelerator is applied to reduce such latency \cite{reagen2021cheetah}, however, specified hardware demand limits generality of the method and further application scope.  

% Recently, A few attempts \cite{roy2019mitigating,singh2021disco} have been made to address the feature leakage problem with Adversarial Representation Learning (ARL).The central idea in these methods contains two parties; 1) an adversarial network aiming to maximize the extraction of sensitive information from a given representation and 2) a task network intending to predict a assigned label with optimal accuracy while preventing leakage of sensitive attribute. Although prevailing performance can be achieved to protect the user private information, the complexity and redundancy incurred by additional adversarial network in ARL-based frameworks may lead to inefficiency and improvability, especially when deploying on resource-hunger scenarios. Furthermore, none of these methods consider attributes leakage during training phase, which is likely occurred to a large extent in the real-world scene.   

% \subsection{Threat Model}
% In collaborative learning, each individual client is susceptible to feature leakage attacks because each client is the participant
% sending itself intermediate activations to the server.
% %
% We assume that the server is an honest-but-curious server with the goal of uncovering the local sensitive features of clients.
% %
% Specially, the server will honestly perform the training on intermediate activations and manage the iteration rounds for collaborative learning. 
% %
% However, the server may be curious and may analyze periodic intermediate activations from certain clients to perform the feature leakage attacks and gain access to the sensitive features of the victim clients.
% %
% It is worth noting that even if the network connection between the client and server is secure, the feature leakage attacks can take place.
